Joint Caching, Routing, and Channel Assignment for Collaborative Small-Cell Cellular Networks

We consider joint caching, routing, and channel assignment for video delivery over coordinated small-cell cellular systems of the future Internet. We formulate the problem of maximizing the throughput of the system as a linear program in which the number of variables is very large. To address channel interference, our formulation incorporates the conflict graph that arises when wireless links interfere with each other due to simultaneous transmission. We utilize the column generation method to solve the problem by breaking it into a restricted master subproblem that involves a select subset of variables and a collection of pricing subproblems that select the new variable to be introduced into the restricted master problem, if that leads to a better objective function value. To control the complexity of the column generation optimization further, due to the exponential number of independent sets that arise from the conflict graph, we introduce an approximation algorithm that computes a solution that is within $\epsilon$ to optimality, at much lower complexity. Our framework demonstrates considerable gains in average transmission rate at which the video data can be delivered to the users, over the state-of-the-art Femtocaching system, of up to 46%. These operational gains in system performance map to analogous gains in video application quality, thereby enhancing the user experience considerably.

==> comcom.tex <==

\usepackage{amsmath, amsfonts, amssymb}
\usepackage{algorithm, algorithmic}
\usepackage{graphicx, comment}
\usepackage{color,subfigure}

% General functions
\def\Rank{\mathop{\rm Rank}\limits}
\def\Zmodm{{\mathbb{Z}}_m}
\def\GF{\mathop{\sf GF}\limits}
\def\bigorder{{\mathcal{O}}}
\def\LB{{\mathrm{LB}}}
\def\UB{{\mathrm{UB}}}
\def\const{{\mathsf{const}}}
\def\mod{\mbox{~mod~}}
\def\deg{{\mathsf{deg}}}
\def\bis{\bfseries\itshape\sffamily}
\def\bir{\bfseries\itshape\rmfamily}
\def\mbir{\bfseries\mathit\rmfamily}
\def\tran{\mathrm{T}}
\def\rank{\mathrm{Rank}}
\def\eg{e.g.\ }
\def \poly{{\mathsf{Poly}}}
\def\diag{{\mathsf{diag}}}
\def\mcmf{{\mathsf{mcmf}}}
\def\head{\mathsf{head}}
\def\tail{\mathsf{tail}}
\def\adj{\mathrm{adj}}




% Common notations
\def\A{{\mathbf{A}}}
\def\E{{\mathbf{E}}}
\def\H{{\mathbf{H}}}
\def\I{{\mathbf{I}}}
\def\M{{\mathbf{M}}}
\def\N{{\mathbf{N}}}
\def\SS{{\mathbf{S}}}
\def\T{{\mathbf{T}}}
\def\X{{\mathbf{X}}}
\def\Y{{\mathbf{Y}}}
\def\a{{\mathbf{a}}}
\def\b{{\mathbf{b}}}
\def\c{{\mathbf{c}}}
\def\d{{\mathbf{d}}}
\def\m{{\mathbf{m}}}
\def\n{{\mathbf{n}}}
\def\q{{\mathbf{q}}}
\def\vv{{\mathbf{v}}}
\def\u{{\mathbf{u}}}
\def\vv{{\mathbf{v}}}
\def\s{{\mathbf{s}}}
\def\t{{\mathbf{t}}}
\def\x{{\mathbf{x}}}
\def\y{{\mathbf{y}}}
\def\0{{\mathbf{0}}}
\def\1{{\mathbf{1}}}
\def\RR{{\mathbb{R}}}
\def\NN{{\mathbb{N}}}
\def\PP{{\mathsf{P}}}
\def\EE{{\mathsf{E}}}

% useful command shorthand
\def\lmat{\left(\begin{matrix}}
\def\rmat{\end{matrix}\right)}
\def\eqref#1{(\ref{#1})}
\def \Definition#1{{\it Definition~#1}}
\def \Definitions#1{{\it Definitions~#1}}
\def \Theorem#1{{Theorem~#1}}
\def \Theorems#1{{Theorems~#1}}
\def \Corollary#1{{\it Corollary~#1}}
\def \Corollaries#1{{\it Corollaries~#1}}
\def \Cor#1{{Corollary~#1}}
\def \Cors#1{{Corollaries~#1}}
\def \Proposition#1{{Proposition~#1}}
\def \Propositions#1{{Propositions~#1}}
\def \Condition#1{{\sc Condition~#1}}
\def \Conditions#1{{\sc Conditions~#1}}
\def \Conj#1{{\sc Conjecture~#1}}
\def \Conjs#1{{\sc Conjectures~#1}}
\def \Lemma#1{{Lemma~#1}}
\def \Lemmas#1{{Lemmata~#1}}
\def \Argument#1{{\sc Argument~#1}}
\def \Arguments#1{{\sc Arguments~#1}}
\def \Fig#1{{Fig.~#1}}
\def \Figs#1{{Figs.~#1}}
\def \Figure#1{{Fig.~#1}}
\def \Figures#1{{Figs.~#1}}
\def \Table#1{{Table~#1}}
\def \Tables#1{{Tables~#1}}
\def \Append#1{{Appendix~#1}}
\def \Appends#1{{Appendice.~#1}}
\def\Algorithm#1{{Algorithm~#1}}
\newenvironment{thmproof}[1]
{\noindent\hspace{2em}{\it #1 }}
{\hspace*{\fill}~\QED\par\endtrivlist\unskip}
\def\subsub#1{{\par \vspace{.25cm} \noindent {\em #1}\par \vspace{.1cm}}}
%\def\subsub#1{{\par \vspace{.25cm} \noindent {\it #1}\par \vspace{.1cm}}}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{condition}{Condition}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{conj}{Conjecture}

% Colors
\def\cb#1{{\color{blue}{#1}}}
\def\cg#1{{\color{green}{#1}}}
\def\clg#1{{\color{lightgray}{#1}}}
\def\cgr#1{{\color{gray}{#1}}}
\def\cbk#1{{\color{black}{#1}}}
\def\cre#1{{\color{red}{#1}}}
\def\cm#1{{\color{magenta}{#1}}}
\def\cy#1{{\color{yellow}{#1}}}
\def\ccy#1{{\color{cyan}{#1}}}


% paper-specific notations
\def\SSS{{\mathbf{S}}}% Set of stopping set
\def\TS#1{{\mathbf{s}^{(#1)}}}% stopping set
\def \ds{{d_{\mathrm{s}}}}
\def \ms{{m_{\mathrm{s}}}}
\newcommand{\Dsup}{{W_{{\mathrm{sup}}}}}
\newcommand{\Ms}{{M_{{\mathrm{s}}}}}
\newcommand{\Dstp}{{D_{{\mathrm{stp}}}}}
\def\Dtrp#1{{D_{{\mathrm{trp}},#1}}}
\def\Mt#1{{M_{{\mathrm{t}},#1}}}
\def\eb{{\#E_{\mathrm{B}}}}
\def\cb{{\#C_{\mathrm{B}}}}
\def\cbodd{{\#C_{\mathrm{B,odd}}}}
\def\vb{{\#V_{\mathrm{B}}}}
\def\lft{{K}}
\def\FERavg{{\mbox{FER}_{\mathrm{avg}}}}
\def\FER{{\mbox{FER}}}
\def \dt#1{{d_{{\mathrm{t}},{#1}}}}
\def \dist{{\mathsf{dist}}}
\def\NCodd{{\#C_{\mathrm{odd}}}}
\def\NCoddT{{\#C_{\mathrm{odd},\geq 3}}}
\def\NCeven{{\#C_{\mathrm{even}}}}
\def\NCevenF{{\#C_{\mathrm{even},\geq 4}}}
\def\Xmod{{{\mathbf{x}}_{\mathrm{o.d.}}}}
\def \Out{{\mathrm{Out}}}
\def \In{{\mathrm{In}}}



% Pictures,
% macro for check nodes
%\def\picchk{\put(-15,-15){\framebox(30,30){}}\put(0,0){\makebox(0,0){\small$+$}}}
\def\picchk{\put(0,0){\circle{30}}\put(0,0){\makebox(0,0){$+ $}}}
% macro for var nodes
\def\picvar{\put(0,0){\circle{30}}\put(0,0){\makebox(0,0){$\bullet$}}}


% Slides
\def\ccmathhl#1{\colorbox{lightyellow}{$#1$}\hspace{-.15cm}} % chihw's math highlight
\def\cchl#1{\colorbox{lightyellow}{#1}} % chihw's math highlight


\def\yca{{\mathsf{yca}}}
\def\EXS{{\mathrm{EXS}}}
\def\DE{{\mathsf{DE}}}
\def\CB{{\mathsf{CB}}}
\def\out{{\mathrm{out}}}
\def\picvar{\put(0,0){\circle{30}}\put(0,0){\makebox(0,0){$\bullet$}}}
\def\picvare#1{\put(0,0){\circle{30}}\put(0,0){\makebox(0,0){#1}}}
\def\picchk{\put(-15,-15){\framebox(30,30){}}\put(0,0){\makebox(0,0){\small$+$}}}
\def\picvara#1{\put(0,0){\circle{30}}\put(0,-3){\makebox(0,0){\scriptsize{#1}}}}
\def\picvarb#1{\put(-45,0){\vector(1,0){30}}\put(0,0){\circle{30}}\put(0,-3){\makebox(0,0){\scriptsize {#1}}}}
%\def\picchka{\put(-15,-15){\line(1,0){30}}\put(-15,15){\line(1,0){30}}\put(15,-15){\line(0,1){30}}\put(-15,-15){\line(0,1){30}}}
\def\picchka{\put(-15,-15){\framebox(30,30){+}}}
%\def\diam#1{\put(-25,0){\line(1,1){25}}\put(-25,0){\line(1,-1){25}}\put(25,0){\line(-1,1){25}}\put(25,0){\line(-1,-1){25}}
%\put(0,0){\makebox(0,0){#1}}}
\def\diam#1{\put(-40,-25){\framebox(80,50){#1}}}


==> comcom1.tex <==

%\usepackage{tabularx}
%\usepackage{booktabs}
%\usepackage{pmat}

%\usepackage{multirow}
%\renewcommand{\multirowsetup}{\centering}


\usepackage{amsmath, amsfonts, amssymb}
\usepackage{algorithm, algorithmic}
\usepackage{graphicx, comment}
\usepackage{color,subfigure}

% General functions
\def\Rank{\mathop{\rm Rank}\limits}
\def\Zmodm{{\mathbb{Z}}_m}
\def\GF{\mathop{\sf GF}\limits}
\def\bigorder{{\mathcal{O}}}
\def\LB{{\mathrm{LB}}}
\def\UB{{\mathrm{UB}}}
\def\const{{\mathsf{const}}}
\def\mod{\mbox{~mod~}}
\def\deg{{\mathsf{deg}}}
\def\bis{\bfseries\itshape\sffamily}
\def\bir{\bfseries\itshape\rmfamily}
\def\mbir{\bfseries\mathit\rmfamily}
\def\tran{\mathrm{T}}
\def\eg{e.g.\ }
\def \poly{{\mathsf{Poly}}}
\def\diag{{\mathsf{diag}}}
\def\co{{\mathrm{Co}}}
\def \Out{{\mathrm{Out}}}
\def \In{{\mathrm{In}}}
\def\head{{\mathrm{head}}}
\def\tail{{\mathrm{tail}}}



% Common notations
\def\A{{\mathbf{A}}}
\def\E{{\mathbf{E}}}
\def\H{{\mathbf{H}}}
\def\I{{\mathbf{I}}}
\def\M{{\mathbf{M}}}
\def\N{{\mathbf{N}}}
\def\S{{\mathbf{S}}}
\def\T{{\mathbf{T}}}
\def\X{{\mathbf{X}}}
\def\Y{{\mathbf{Y}}}
\def\c{{\mathbf{c}}}
\def\m{{\mathbf{m}}}
\def\n{{\mathbf{n}}}
\def\q{{\mathbf{q}}}
\def\u{{\mathbf{u}}}
\def\v{{\mathbf{v}}}
\def\r{{\mathbf{r}}}
\def\s{{\mathbf{s}}}
\def\t{{\mathbf{t}}}
\def\w{{\mathbf{w}}}
\def\x{{\mathbf{x}}}
\def\y{{\mathbf{y}}}
\def\0{{\mathbf{0}}}
\def\1{{\mathbf{1}}}
\def\RR{{\mathbb{R}}}
\def\NN{{\mathbb{N}}}
\def\PP{{\mathsf{P}}}
\def\EE{{\mathsf{E}}}

% useful command shorthand
\def\lmat{\left(\begin{matrix}}
\def\rmat{\end{matrix}\right)}
\def\eqref#1{(\ref{#1})}
\def \Definition#1{{\it Definition~#1}}
\def \Definitions#1{{\it Definitions~#1}}
\def \Theorem#1{{Theorem~#1}}
\def \Theorems#1{{Theorems~#1}}
\def \Corollary#1{{\it Corollary~#1}}
\def \Corollaries#1{{\it Corollaries~#1}}
\def \Cor#1{{Corollary~#1}}
\def \Cors#1{{Corollaries~#1}}
\def \Proposition#1{{Proposition~#1}}
\def \Propositions#1{{Propositions~#1}}
\def \Condition#1{{\sc Condition~#1}}
\def \Conditions#1{{\sc Conditions~#1}}
\def \Conj#1{{\sc Conjecture~#1}}
\def \Conjs#1{{\sc Conjectures~#1}}
\def \Lemma#1{{Lemma~#1}}
\def \Lemmas#1{{Lemmata~#1}}
\def \Argument#1{{\sc Argument~#1}}
\def \Arguments#1{{\sc Arguments~#1}}
\def \Fig#1{{Fig.~#1}}
\def \Figs#1{{Figs.~#1}}
\def \Figure#1{{Fig.~#1}}
\def \Figures#1{{Figs.~#1}}
\def \Table#1{{Table~#1}}
\def \Tables#1{{Tables~#1}}
\def \Append#1{{Appendix~#1}}
\def \Appends#1{{Appendice.~#1}}
\def\Algorithm#1{{Algorithm~#1}}
\newenvironment{thmproof}[1]
{\noindent\hspace{2em}{\it #1 }}
{\hspace*{\fill}~\QED\par\endtrivlist\unskip}
\def\subsub#1{{\par \vspace{.25cm} \noindent {\it #1}\par \vspace{.1cm}}}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{condition}{Condition}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{conj}{Conjecture}
\newtheorem{inequality}{Inequality}


% Colors
\def\cb#1{{\color{blue}{#1}}}
\def\cg#1{{\color{green}{#1}}}
\def\clg#1{{\color{lightgray}{#1}}}
\def\cgr#1{{\color{gray}{#1}}}
\def\cbk#1{{\color{black}{#1}}}
\def\cre#1{{\color{black}{#1}}}
\def\cm#1{{\color{magenta}{#1}}}
\def\cy#1{{\color{yellow}{#1}}}
\def\ccy#1{{\color{cyan}{#1}}}


% paper-specific notations
\def\SS{{\mathbf{s}}}% stopping set
\def\SSS{{\mathbf{S}}}% Set of stopping set
\def\TS#1{{\mathbf{s}^{(#1)}}}% stopping set
\def \ds{{d_{\mathrm{s}}}}
\def \ms{{m_{\mathrm{s}}}}
\newcommand{\Dsup}{{W_{{\mathrm{sup}}}}}
\newcommand{\Ms}{{M_{{\mathrm{s}}}}}
\newcommand{\Dstp}{{D_{{\mathrm{stp}}}}}
\def\Dtrp#1{{D_{{\mathrm{trp}},#1}}}
\def\Mt#1{{M_{{\mathrm{t}},#1}}}
\def\eb{{\#E_{\mathrm{B}}}}
\def\cb{{\#C_{\mathrm{B}}}}
\def\cbodd{{\#C_{\mathrm{B,odd}}}}
\def\vb{{\#V_{\mathrm{B}}}}
\def\lft{{K}}
\def\FERavg{{\mbox{FER}_{\mathrm{avg}}}}
\def\FER{{\mbox{FER}}}
\def \dt#1{{d_{{\mathrm{t}},{#1}}}}
\def \dist{{\mathsf{dist}}}
\def\NCodd{{\#C_{\mathrm{odd}}}}
\def\NCoddT{{\#C_{\mathrm{odd},\geq 3}}}
\def\NCeven{{\#C_{\mathrm{even}}}}
\def\NCevenF{{\#C_{\mathrm{even},\geq 4}}}
\def\Xmod{{{\mathbf{x}}_{\mathrm{o.d.}}}}



% Pictures,
% macro for check nodes
%\def\picchk{\put(-15,-15){\framebox(30,30){}}\put(0,0){\makebox(0,0){\small$+$}}}
\def\picchk{\put(0,0){\circle{30}}\put(0,0){\makebox(0,0){$+ $}}}
% macro for var nodes
\def\picvar{\put(0,0){\circle{30}}\put(0,0){\makebox(0,0){$\bullet$}}}


% Slides
\def\ccmathhl#1{\colorbox{lightyellow}{$#1$}\hspace{-.15cm}} % chihw's math highlight
\def\cchl#1{\colorbox{lightyellow}{#1}} % chihw's math highlight


\def\yca{{\mathsf{yca}}}
\def\EXS{{\mathrm{EXS}}}
\def\DE{{\mathsf{DE}}}
\def\CB{{\mathsf{CB}}}
\def\out{{\mathrm{out}}}
\def\picvar{\put(0,0){\circle{30}}\put(0,0){\makebox(0,0){$\bullet$}}}
\def\picvare#1{\put(0,0){\circle{30}}\put(0,0){\makebox(0,0){#1}}}
\def\picchk{\put(-15,-15){\framebox(30,30){}}\put(0,0){\makebox(0,0){\small$+$}}}
\def\picvara#1{\put(0,0){\circle{30}}\put(0,-3){\makebox(0,0){\scriptsize{#1}}}}
\def\picvarb#1{\put(-45,0){\vector(1,0){30}}\put(0,0){\circle{30}}\put(0,-3){\makebox(0,0){\scriptsize {#1}}}}
%\def\picchka{\put(-15,-15){\line(1,0){30}}\put(-15,15){\line(1,0){30}}\put(15,-15){\line(0,1){30}}\put(-15,-15){\line(0,1){30}}}
\def\picchka{\put(-15,-15){\framebox(30,30){+}}}
%\def\diam#1{\put(-25,0){\line(1,1){25}}\put(-25,0){\line(1,-1){25}}\put(25,0){\line(-1,1){25}}\put(25,0){\line(-1,-1){25}}
%\put(0,0){\makebox(0,0){#1}}}
\def\diam#1{\put(-40,-25){\framebox(80,50){#1}}}






\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

